Soundness-Aware Level: A Microscopic Signature that Predicts LLM Reasoning Potential

Reinforcement learning with verifiable rewards (RLVR) can elicit strong reasoning in large language models (LLMs), while their performance after RLVR varies dramatically across different base models. This raises a fundamental question: what microscopic property of pre-trained models leads to this variation? To investigate, we formalize reasoning as chains of Horn clauses ("if-then" rules) built from features extracted from the LLM's latent space via cross-layer sparse autoencoders (SAEs). We estimate the transition probabilities between its features, and further categorize each rule by its semantic soundness level (e.g., strict, plausible, noisy) with an LLM. Our key discovery is that high-potential models are inherently soundness-aware: their internal probability distributions systematically shift across rules' soundness levels, becoming highly distinct for "strict" versus "noisy" rules. In contrast, weaker models are soundness-agnostic, collapsing to one distribution regardless of soundness levels. To quantify this, we introduce the Soundness-Aware Level (SAL), a microscopic metric using the Jensen-Shannon Divergence to measure the separation between these distributions. We show that SAL's predictions of post-RLVR reasoning performance follow a precise empirical law (R^2=0.87) across diverse model families (Qwen, Mistral, Llama, DeepSeek) and scales (0.5B-14B). This reveals that a model's reasoning potential is tied to its intrinsic, pre-trained ability to distinguish sound knowledge from unsound ones. These findings underscore the critical role of model pre-training in shaping reasoning and offer a practical metric grounded in the model's internal mechanisms for selecting/designing stronger base models.

==> __bak_experiment.tex <==
\section{Analysis}
\label{sec:analysis}
This section empirically answers three research questions (RQs). 
RQ1: What are the microscopic differences between models with and without strong reasoning potentials, and can the proposed metric in Section~\ref{sec:metric} quantify these differences?
RQ2: Can the proposed metric effectively reveal the reasoning potential of different LLMs?
RQ3: How do various factors (i.e., model scale and model family) affect these internal differences?

\subsection{General Settings}
\label{settings}
\paragraph{Datasets.} 
Following previous research that focuses on the mathematical solving task to analyze the reasoning capabilities of LLMs, we construct our training dataset by selecting mathematical problems from various resources. 
Specifically, we consider the full Math~\citep{hendrycks2measuring} dataset, Open Reasoner Zero~\citep{hu2025open}, GSM8K~\citep{cobbe2021gsm8k}, and the AOPS, AMC, and Olympiad subsets from the NuminaMath~\citep{numina_math_datasets}. 
These datasets cover various mathematical topics across different difficulty levels, starting from a straightforward application of calculation (e.g., GSM8K) to competition-level questions (e.g., Olympiad). 
By de-duplicating samples, the dataset includes 128K unique questions with an average of 81.42 tokens per question. 
Following previous research~\citep{deepseek2025r1,hu2025open}, each candidate LLM will be prompted to generate one response to each question, formatted by a ``think'' included in a conversational template. 
The cross-layer SAE for each candidate LLM will be trained on the corpus consisting of both the prompting questions and their own generated responses. 
%Finally, we collect a total of 102M tokens for SAE training.



\paragraph{Language Models.} 
Our analysis concentrates on the pre-trained \texttt{Qwen-2.5-7B}~~\citep{hui2024qwen2} as our main subject model, as it has demonstrated superior performance on various reasoning tasks. We also include the pre-trained \texttt{Qwen-2.5-0.5B}, \texttt{Qwen-2.5-1.5B}, and \texttt{Qwen-2.5-14B} to study the impact of \textbf{model scale} on our conclusions. In addition, we consider \texttt{Mistral-7B-v0.1}~\citep{jiang2023mistral7b}, \texttt{Llama-3.1-8B}~\citep{dubey2024llama}, and \texttt{DeepSeek-Math-7B}~\cite{shao2024deepseekmath} to examine the impact of \textbf{model family}. 


\pgfplotsset{
  mybars/.style={
    ybar, bar width=4pt,
    fill opacity=.25, draw opacity=.8,
    tick style={draw=none},
    mark=none
  },
  myaxis/.style={
    width=.4\textwidth, height=.3\textwidth,
    xmin=0, xmax=1, ymin=0, ymax=.27,
    xtick={0,.2,...,1}, ytick={0,.1,.2},
    axis line style={thin}, tick style={thin},
    ymajorgrids,
    title style={yshift=-.6ex},      % subtitle tight
    xticklabel style={font=\tiny},
    tick style={draw=none},
    yticklabel style={font=\tiny}
  }
}



\paragraph{Training Cross-Layer SAEs.}
Following previous research~\citep{jack2024sparse}, we train our SAEs on the residual stream of the subject LLMs. 
For a comparable analysis on extracted features across different models, different subject LLMs share the same SAE structure with the number of features $C=2^{15}$ and the total number of layers $L=8$. 
We select $L$ layers as evenly as possible. For example, for the \texttt{Qwen-2.5-1.5B/7B} models with a total of 28 layers, we monitor every 4 layers, where the first time of monitoring is the inputs of the first layer.
Following recommendations by~\citet{gaoscaling}, we apply AdamW~\citep{loshchilov2017decoupled} optimizer with $\beta_1=0.9$, $\beta_2=0.999$, and $\epsilon=6.25e^{-10}$ to train crosscoders using an initialized learning rate $2e^{-4}$ with a cool down strategy in the last 20\% steps as suggested by~\cite{jack2024sparse}. 
The default sparse penalty $\alpha$ is $5e^{-3}$ with a linear warm-up strategy over the first 20\% steps. 
To this end, the trained crosscoders achieve a normalized MSE of around 0.65-0.80, with an average of 20-30 activated features, to reconstruct each token. 
More details can be found in Appendix~\ref{appd:SAE}.


\paragraph{Machine Annotation.} 
To perform our analysis on the extracted logic rules, we scale up the annotation process of classifying each rule into one of the types from ``No'', ``Plausible'', and ``Strict'' with machine annotators. 
Previous research~\citep{autoscale,bills2023language,gaoscaling} has shown that modern LLMs can provide faithful explanations of the features according to their most activated text spans. 
We follow their path and further prompt an LLM to judge which type the extracted logic rule belongs to, according to the textual feature explanations thoroughly. 
For the best precision, we deploy DeepSeek-R1~\citep{guo2025deepseek} to serve as our machine annotator. 
We report more detailed settings, and the results of reliability analysis in the Appendix~\ref{appd:interpret_SAE} and Appendix~\ref{apd:rule_extract}.


\subsection{RQ1: Micro Differences between Strong and Weak Reasoning Models}
\label{finding1}
\label{finding_one}



\begin{figure*}
\centering
\footnotesize
\begin{tikzpicture}

  %---------------- GROUPPLOT (3 columns × 2 rows) -----------------
  \begin{groupplot}[
    group style={
      group size=3 by 2,
      horizontal sep=0.2cm,      % breathing room
      vertical sep=.3cm
    },
    myaxis,
    every axis plot/.append style={mybars}
  ]

  % ---------- ROW 1 : STRONG (Qwen) ---------------------------------
  \nextgroupplot[xticklabels=\empty]
     \addplot[fill=blue!40]  coordinates {
      (0.025,0.0000) (0.07500000000000001,0.0668) (0.125,0.2038) (0.17500000000000002,0.0356) (0.225,0.0367) (0.275,0.0624) (0.32500000000000007,0.0379) (0.37500000000000006,0.0256) (0.42500000000000004,0.0045) (0.47500000000000003,0.0011) (0.525,0.0000) (0.5750000000000001,0.0011) (0.6250000000000001,0.0145) (0.675,0.0256) (0.7250000000000001,0.1314) (0.775,0.0869) (0.8250000000000001,0.0401) (0.8750000000000001,0.0724) (0.925,0.1347) (0.9750000000000001,0.0189)
    };

  \nextgroupplot[yticklabels=\empty,  xticklabels=\empty]
     \addplot[fill=blue!40]   coordinates {
      (0.025,0.0000) (0.07500000000000001,0.0876) (0.125,0.1969) (0.17500000000000002,0.0269) (0.225,0.0587) (0.275,0.1568) (0.32500000000000007,0.0864) (0.37500000000000006,0.0400) (0.42500000000000004,0.0113) (0.47500000000000003,0.0038) (0.525,0.0003) (0.5750000000000001,0.0028) (0.6250000000000001,0.0086) (0.675,0.0176) (0.7250000000000001,0.0383) (0.775,0.0385) (0.8250000000000001,0.0521) (0.8750000000000001,0.1030) (0.925,0.0645) (0.9750000000000001,0.0060)
    };

  \nextgroupplot[yticklabels=\empty,  xticklabels=\empty]
     \addplot[fill=blue!40] coordinates {
      (0.025,0.0000) (0.07500000000000001,0.0462) (0.125,0.0769) (0.17500000000000002,0.0462) (0.225,0.0154) (0.275,0.0462) (0.32500000000000007,0.0769) (0.37500000000000006,0.0769) (0.42500000000000004,0.0308) (0.47500000000000003,0.0000) (0.525,0.0154) (0.5750000000000001,0.0000) (0.6250000000000001,0.0000) (0.675,0.0000) (0.7250000000000001,0.0000) (0.775,0.0615) (0.8250000000000001,0.1692) (0.8750000000000001,0.2308) (0.925,0.1077) (0.9750000000000001,0.0000)
    };

  

  % ---------- ROW 2 : WEAK (Llama) ----------------------------------
  \nextgroupplot[]
     \addplot[fill=red!40]  coordinates {
      (0.025,0.0000) (0.07500000000000001,0.0000) (0.125,0.0000) (0.17500000000000002,0.0015) (0.225,0.0058) (0.275,0.0087) (0.32500000000000007,0.0087) (0.37500000000000006,0.0044) (0.42500000000000004,0.0073) (0.47500000000000003,0.0044) (0.525,0.0073) (0.5750000000000001,0.0290) (0.6250000000000001,0.0421) (0.675,0.0421) (0.7250000000000001,0.0581) (0.775,0.1118) (0.8250000000000001,0.1800) (0.8750000000000001,0.1684) (0.925,0.0900) (0.9750000000000001,0.2308)
    };

  \nextgroupplot[yticklabels=\empty]
     \addplot[fill=red!40]   coordinates {
      (0.025,0.0000) (0.07500000000000001,0.0000) (0.125,0.0000) (0.17500000000000002,0.0020) (0.225,0.0104) (0.275,0.0050) (0.32500000000000007,0.0084) (0.37500000000000006,0.0062) (0.42500000000000004,0.0042) (0.47500000000000003,0.0127) (0.525,0.0152) (0.5750000000000001,0.0251) (0.6250000000000001,0.0373) (0.675,0.0333) (0.7250000000000001,0.0410) (0.775,0.0581) (0.8250000000000001,0.1888) (0.8750000000000001,0.2487) (0.925,0.1250) (0.9750000000000001,0.1786)
    };
    
  \nextgroupplot[yticklabels=\empty]
     \addplot[fill=red!40] coordinates {
      (0.025,0.0000) (0.07500000000000001,0.0000) (0.125,0.0000) (0.17500000000000002,0.0134) (0.225,0.0179) (0.275,0.0223) (0.32500000000000007,0.0134) (0.37500000000000006,0.0045) (0.42500000000000004,0.0000) (0.47500000000000003,0.0134) (0.525,0.0089) (0.5750000000000001,0.0223) (0.6250000000000001,0.0179) (0.675,0.0045) (0.7250000000000001,0.0313) (0.775,0.0402) (0.8250000000000001,0.1920) (0.8750000000000001,0.2589) (0.925,0.1964) (0.9750000000000001,0.1429)
    };

    

  \end{groupplot}
  \node[rotate=270,font=\bfseries] at ($(group c3r1.east)+(0.3cm,0)$) {Stronger};
  \node[rotate=270,font=\bfseries] at ($(group c3r2.east)+(0.3cm,0)$) {Weaker};
  \node[] at ($(group c2r2.south)+(0.0cm,-0.5cm)$) {Probability $\hat{p}(C|P)$};
  \node[rotate=90] at ($(group c1r1.north)!0.5!(group c1r2.south)+(-2.8cm,0cm)$) {Frequency};

  %----------------- COLUMN HEADERS (rule types) --------------------
  \node[font=\bfseries,anchor=south]
        at ($(group c1r1.north)+(0,0.cm)$) {``No'' Logic Rule};
  \node[font=\bfseries,anchor=south]
        at ($(group c2r1.north)+(0,0.cm)$) {``Plausible'' Logic Rule};
  \node[font=\bfseries,anchor=south]
        at ($(group c3r1.north)+(0,0.cm)$) {``Strict'' Logic Rule};

\end{tikzpicture}
\caption{Probability distribution of extracted logic rules from a pair of stronger (\texttt{Qwen‑2.5‑7B}) and weaker (\texttt{Llama‑3.1‑8B}) models. Within each row, the stronger model shows significant different distributions for No, Plausible, and Strict logic rules, whereas the weaker model collapse toward similar shapes, indicating a failure of recognizing different types of logic rules.}
\label{fig:logic-rule-dists}
\end{figure*}

\paragraph{Finding 1: Stronger models discriminate sharply between strict, plausible, and noisy rules, whereas weaker models collapse these categories into an almost indistinguishable distribution.}
In Figure~\ref{fig:logic-rule-dists}, the strong \texttt{Qwen-2.5-7B} exhibits three qualitatively different histograms: ``Strict'' rules cluster tightly at high probabilities, ``Plausible'' rules form a broad mid-range shoulder, and ``No'' rules gather mostly near zero with a small tail at higher values. 
By contrast, the weak \texttt{Llama-2.5-8B} shows nearly identical right-skewed shapes for all three labels, with most mass above $75\%$. 
This inability to keep noisy and heuristic clauses apart from genuinely strict ones suggests that the weaker model treats many co-activations as equally reliable, blurring the logical boundaries that a more capable reasoner maintains. 
The qualitative gap motivates our hypothesis that internal rule-type separability is a hallmark of reasoning strength, a claim we quantify with the divergence-based metric introduced in Section \ref{sec:metric} and validate in the subsequent analyses.



% \begin{wraptable}{r}{7.5cm}
% \vspace{-0.4cm}
% \centering
% \small
% \caption{JSD quantifies distribution shifts between rule types (S: ``Strict'', P: ``Plausible'', \& N: ``No'').}
% \vspace{-0.3cm}
% \label{tab:jsd}
% \begin{tabular}{lcccc}
% \toprule
% \toprule
% $\textbf{Model}$ & $\textbf{S vs. P}$ & $\textbf{S vs. N}$ & $\textbf{P vs. N}$ & $\textbf{S vs. P vs. N}$ \\
% \midrule
% Qwen  & 0.111 & 0.162 & 0.068 & 0.201 \\
% Llama & 0.020 & 0.042 & 0.012 & 0.058 \\
% \bottomrule
% \bottomrule
% \end{tabular}
% \vspace{-0.4cm}
% \end{wraptable}
\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-0.3cm}
\includegraphics[width=1.0\linewidth]{figures/Figure_4.pdf}
\caption{Jensen-Shannon Divergence (JSD) quantifies distribution shifts between probabilities of soundness levels (S: ``Strict'', P: ``Plausible'', \& N: ``No'').}
\label{fig:jsd_barplot}
\vspace{-0.4cm}
\end{wrapfigure}
\paragraph{Finding 2: Jensen-Shannon Divergence (JSD) can quantify the differences between the probability distributions from different groups.}
To validate the qualitative distinctions observed in Figure~\ref{fig:logic-rule-dists}, we apply the divergence-based metric introduced in Section~\ref{sec:metric} to measure how well each model separates the three types of logic rules. As shown in Figure~\ref{fig:jsd_barplot}, the stronger model (\texttt{Qwen-2.5-7B}) achieves substantially higher Jensen-Shannon divergences across all rule pairs: $0.111$ for Strict vs. Plausible, $0.162$ for Strict vs. No, and $0.068$ for Plausible vs. No, resulting in an overall JS-divergence of $0.201$. In contrast, the weaker one (\texttt{Llama-2.5-8B}) yields much smaller values in all categories, with overall JS-Divergence at $0.058$. These results confirm that JSD effectively quantifies the results of qualitative analysis presented in Finding 1. 
%Moreover, the observed numerical differences align with the visual differences in histogram shape, reinforcing that strong reasoning models not only encode richer structure but also represent it in ways that can be reliably measured.



\begin{figure*}
    \centering
    \includegraphics[width=0.49\linewidth ]{figures/Figure_1.pdf}
    \includegraphics[width=0.49\linewidth]{figures/Figure_3.pdf}
    \caption{Left: Correlation between the SAL over extracted rules and models' post-RLVR performance. Right: The exponential power law $\epsilon=\exp(-\alpha\cdot s^{\,\beta})$ describes the correlation between SAL $s$ and the error rate $\epsilon$ of solving mathematical problems. The best fitted model is $\alpha = 4.246$ and $\beta = 1.090$ with $R^{2}=0.985$ for interpolation fitting observed models.}
  \label{fig:qualitative-corr-main}
\end{figure*}


\subsection{RQ2: Correlation between Microscopic Signature and Reasoning Abilities}

\paragraph{Finding 3: Higher Soundness-Aware Level tightly tracks higher reasoning accuracy.}
Figure~\ref{fig:qualitative-corr-main} (left) plots normalized JS-Divergence against the average accuracy of seven checkpoints. The points fall almost exactly on an exponential‐like curve with $R^{2}=0.984$, indicating an extremely strong monotonic relationship. When the JS-Divergence is near zero, accuracy hovers around 5\%. As the score rises to roughly 0.35, accuracy more than doubles, and at a JS-Divergence close to 1 the model reaches about 41\% accuracy. This pattern shows that the proposed micro-level metric captures the macroscopic improvement in reasoning: larger separations in the learned feature distributions coincide with markedly better performance on the mathematical task.

% \paragraph{Finding 4: The correlation between JS-Divergence and post-RL performance persists across diverse benchmarks.}
% Table~\ref{tab:correlation} quantifies the observation on the monotonic relationship by measuring the Spearman correlations between various predictors and post-training accuracy. JS-Divergence attains at least 89\% on every dataset and averages 96.4\%, outperforming behavioral counts, pre-RL baseline scores on the GSM8K dataset. This consistency across tasks of different formats and difficulty levels confirms that JS-Divergence is a reliable, model-agnostic indicator of reasoning strength, whereas competing metrics exhibit weaker or uneven correlations.


\paragraph{Finding 4: SAL offers a robust and mechanistically-grounded signature of reasoning potential.}
Table~\ref{tab:correlation} reports the Spearman correlation between various predictors. For the baselines based on counting the frequency of varied cognitive behaviors, we follow the protocols~\citep{yue2025does} to extract those behaviors shown on our same dataset to ensure comparability with us. Our SAL metric is a consistently strong predictor, averaging 96.4\% correlation and outperforming most behavioral and pre-RL baselines, except for ``Pre-RL MATH500''. While the ``Pre-RL MATH500'' score is also a powerful predictor, SAL's distinct value lies in its mechanistic insight. Instead of measuring performance on a single task like GSM8K or MATH500, SAL quantifies a model's intrinsic ability to distinguish sound from unsound knowledge internally. This makes it a more fundamental indicator of a model's reasoning signature, explaining its high correlation across diverse benchmarks.






\begin{table*}
\centering
\small
\caption{Spearman correlation (\%) between SAL and model performance after RLVR training. The post RL (GRPO) performances of different base models are referenced from~\cite{zeng2025simplerl}.}
\label{tab:correlation}
%\vspace{-0.2cm}

\begin{tabular}{cc|cccccc}
\toprule
\toprule
 & \textbf{Metric} 
 & \textbf{AMC23} 
 & \textbf{MATH500}
 & \textbf{Minerva} 
 & \textbf{Olympiad} 
 & \textbf{AIME24} 
 & \textbf{Avg. Acc.} \\ \hline

\multicolumn{7}{l}{\small{\textit{\#Behavior}}} \\
&Verification & 96.43 & 85.71 & 75.00 & 85.71 & 77.83  & 85.71 \\
&Backtracking  & 85.71 & 67.86 & 50.00 & 67.86 & 63.01 & 67.86 \\
&Subgoal       & 89.29 & 78.57 & 67.86 & 78.57 & 77.83 & 78.57 \\
&Backward      &  \,\,\,3.60 &  \,\,\,5.41 &  \,\,\,9.01 &  \,\,\,5.41 & 26.18 &  \,\,\,5.41 \\ \midrule

\multicolumn{7}{l}{\small{\textit{Pre-RL Perf.}}} \\
&GSM8K        & 85.71 & 85.71& 75.00 & 85.71 & 81.54  & 85.71 \\
&MATH500      & 92.86 & 100.0& 96.43 & 100.0 & 96.36  & 100.0 \\\midrule

\multicolumn{7}{l}{\small{\textit{Ours}}} \\
&SAL& 89.29 & 96.43 & 92.86 & 96.43 & 96.36  & 96.43 \\
\bottomrule
\bottomrule
\end{tabular}
\end{table*}


\paragraph{Forecasting the correlation between SAL and post-RL performance.} 
We are interested in whether our proposed method can forecast the post-RL performance of a base model. 
To do so, we make two assumptions at the upper and lower bounds of our proposed JS-Divergence metric and fit a curve to model their relationships. 
The theoretical lower bound of the proposed SAL is $\text{SAL}\geq 0.0$, where the model has zero ability to distinguish different types of logic rules, leading to a $100\%$ error rate on the mathematical problems after RL training. 
On the other hand, the theoretical upper bound of SAL is $\text{SAL}\leq\log_2(3)$ in our setting, where the model can precisely distinguish different types of logic rules, enabling it to achieve $0\%$ error rate after RL-training for solving mathematical problems. 
With these two theoretical boundaries, we estimate an empirical law to describe the relation between the SAL and error rate $\epsilon$ as 
\begin{equation}
    \epsilon=\exp(-\alpha\cdot \text{SAL} ^{\beta}),
    \label{eq:scaling_law}
\end{equation}
where $\alpha=4.25$ and $\beta=1.09$, capturing $98.5\%$ of the variance ($R^{2}=0.985$). 
To confirm that our estimated \Eqref{eq:scaling_law} can guide the prediction of reasoning capabilities of future models absent from our experiments, we conduct a leave-one-out validation experiment, where we iteratively remove one interior checkpoint at a time, refit \Eqref{eq:scaling_law} on the remaining eight points while keeping the two boundary anchors, and predict the held-out sample. 
We observe $R^2=0.872$ in this setting, confirming the estimated law generalizes to forecast post-RL performance for unseen base models.


% \begin{figure*}
% \vspace{-0.4cm}
% \centerline{\includegraphics[width=0.65\linewidth]{figures/Figure_3.pdf}}
% \vspace{-0.2cm}
% \caption{The exponential power law $\mathrm{Err}(x)=\exp(-\alpha\,x^{\,\beta})$ describes the correlation between JS-Divergence of and error rate of solving mathematical problems. The best fitted model is $\alpha = 4.246$ and $\beta = 1.090$ with $R^{2}=0.985$.}
% \label{fig:forcasting}
% \vspace{-0.4cm}
% \end{figure*}

\subsection{RQ3: Impacts of Scales and Families on Micro Differences}

\paragraph{Finding 5: Micro‐level differentiation grows monotonically with model scale.}
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \vspace{-0.2cm}
  \includegraphics[width=0.49\textwidth]{figures/Figure_2.pdf}
  \vspace{-0.2cm}
  \caption{Soundness-Aware Level increases with model scale within the Qwen family.}
  \label{fig:scale_comparision}
\vspace{-0.2cm}
\end{wrapfigure}
Figure~\ref{fig:scale_comparision} shows that JS‑Divergence climbs from around 0.06 in the 0.6B checkpoint to around 0.22 from the 14B model, with a clear upward trajectory at every intermediate size. The increase is sharp between 0.5B and 1.5B checkpoints, but becomes moderate beyond that, suggesting a marginal gain in representational separation once sufficient capacity is available. 
If we assume that different scales of Qwen checkpoints share the same training corpus, this monotonic but log-style pattern indicates that simply scaling the parameters further cannot significantly amplify the model's reasoning capabilities, motivating future research to explore more efficient ways for empowering their reasoning capabilities. Beyond 14B, the curve appears close to saturation, indicating that additional parameters may mostly refine existing clusters rather than create new separations in behavior space. In other words, capacity helps the model sort rules more cleanly up to a threshold, then the marginal gains taper. This pattern suggests that architectural or data interventions, such as targeting pre-training on reasoning behaviors or constraining aware objectives, may be more effective than simply scaling up for improving separation.



%\newpage
\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \small
  \vspace{-0.4cm}
  \begin{tikzpicture}
    \begin{axis}[%
        ybar,
        bar width=10pt,
        ylabel={SAL},
        tick style={draw=none},
        symbolic x coords={Qwen,Mistral,Llama,DS-Math},
        xtick=data,
        ymin=0,
        enlarge x limits=0.15,
        height=3.5cm,
        width=0.48\textwidth,
        ymajorgrids,
        ytick={0.05,0.1,0.15},
        yticklabels={0.05,0.1,0.15},
        legend style={at={(0.5,-0.3)},anchor=north,legend columns=-1,draw=none},
    ]
      \addplot+[draw=black,fill=blue!30] coordinates {
        (Qwen,0.1573) (Mistral,0.0644) (Llama,0.0574) (DS-Math,0.1113) 
      };
    \end{axis}
  \end{tikzpicture}
  \vspace{-0.2cm}
  \caption{Comparing soundness-aware level across different model families, where each candidate contains around 7B parameters.}
  \label{fig:model_comparision}
\vspace{-0.4cm}
\end{wrapfigure}
\paragraph{Finding 6: Different model families exhibit distinct microscopic differences.}
Figure~\ref{fig:model_comparision} compares four checkpoints that each hold roughly 7B parameters. The JS-Divergence varies sharply among them: Qwen scores about 0.15, the continue pre-trained DS‑Math reaches roughly 0.11, whereas the general and earlier models like Mistral and Llama models stay near 0.05. Since the parameter count is fixed, these gaps arise from differences in architecture and data selections. The evidence shows that a model’s family leaves a recognizable microscopic signature that either promotes or limits the separation of its learned feature distributions, and by extension its reasoning strength.

\subsection{Case Studies}
Table~\ref{tab:case_study} condenses the logic-rule analysis into four telling snapshots: (i) (i) a strict equivalence rule where the token \texttt{\textbackslash equiv} together with a visible variable $a$ almost deterministically signals an algebraic equation or expression ($p\approx0.977$); (ii) an intermediate procedural reasoning in Example 2, where step-by-step phrases such as ``solve for (x)'' and explanatory markers like ``which'' reliably precede the operation ``divide both sides'' ($p\approx0.896$), reflecting a heuristic grounded in the natural flow of isolating a variable; (iii) a plausible algebraic cue in which the token ``formula'' together with an additive expression typically precedes a concrete numerical value ($p\approx0.846$); and (iv) a noise case that links generic LaTeX delimiters to the phrase ``according to the problem,'' which the model treats as spurious with low confidence ($p\approx0.285$). These observations show that \texttt{Qwen-2.5-7B} can distinguish near-deterministic deductions from useful procedural heuristics and spurious co-occurrences.
Together, these cases show that the proposed framework can identify meaningful logic rules encoded by the models, and trace the model's awareness to their soundness. 


\begin{table*}
    \caption{Examples of extracted logic rules. For each case, we report the model's soundness awareness level $\hat{p}(C|P)$ along with DeepSeek-R1 generated feature explanations ($P_1$, $P_2$, and $C$), the soundness judgments, and justifications for the judgments.}
    \label{tab:case_study}
    \vspace{-0.3cm}
    \centering
    \small
    \begin{tabular}{p{0.01cm}p{0.7cm}|p{12.cm}}
    \toprule
    \toprule
         \multicolumn{3}{l}{\small\textbf{\textit{Example 1:} ``Strict'', $\hat{p}(C|P_1\wedge P_2)=0.9766$}} \\
         &$P_1$&  Pattern "\textbackslash equiv". \\
         &$P_2$&  Pattern "\$a" as a variable (e.g., "length \$a", "integer \$a", "coordinates ... (-a", "2a"). \\
          &$C$&  Algebraic equations and expressions ending with numerical results (e.g., "= 0", "= 16", "\^2"). \\
          &Justify &  Equivalence relations with variable ``a'' imply algebraic equations. \\
          \midrule
         \multicolumn{3}{l}{\small\textbf{\textit{Example 2:} ``Plausible'', $\hat{p}(C|P_1\wedge P_2)=0.8960$}} \\
         
     &$P_1$&  Steps in mathematical problem-solving involving solving/calculating variables or terms, e.g., ``solve for (x)", ``calculate (c)", ``find tan(B)". \\
     &$P_2$&  Pattern ``which" in mathematical explanations (e.g., ``values of (b) for which", ``smallest integer $x$ for which"). \\
      &$C$&  Pattern ``divide both sides". \\
      &Justify &  Using division to isolate variables under conditions. \\
      \midrule 

          \multicolumn{3}{l}{\small\textbf{\textit{Example 3:} ``Plausible'', $\hat{p}(C|P_1\wedge P_2)=0.8461$}} \\
         &$P_1$&  Pattern ``formula". \\
         &$P_2$&  Mathematical expressions with addition in algebraic equations, e.g., ``$x^2$ +", ``x +", ``$ax^3$ +". \\
          &$C$&  Pattern ``Numerical value'' or equation followed by a period (e.g., ``X.", ``Y/Z.", ``= Z\$."). \\
          &Justify &  Algebraic steps with addition may lead to numerical solutions. \\

          \midrule 
          \multicolumn{3}{l}{\small\textbf{\textit{Example 4:} ``No'', $\hat{p}(C|P_1\wedge P_2)=0.2854$}} \\
         &$P_1$&  Start of mathematical expressions/equations in LaTeX, e.g., ``[...", ``\$...", ``sum", ``sqrt", ``frac". \\
         &$P_2$&  Pattern ``\$" indicating LaTeX math mode initiation/termination. \\
          &$C$&  Pattern ``According to the problem". \\
          &Justify &  No logical or heuristic link between LaTeX math and problem reference. \\

          
    \bottomrule
    \bottomrule
    \end{tabular}
    \vspace{-0.5cm}
\end{table*}

% \paragraph{Finding 3: Extracted logic rules from stronger models reflect more advanced problem-solving behaviors, particularly in the verification stage.}
% To explore whether extracted logic rules reflect recognizable stages of mathematical reasoning, we categorize them according to Pólya’s four-step problem-solving framework. Figure~\ref{fig:heuristics-grouped-bar} shows the count of rules aligned with each reasoning step for both \texttt{Qwen-2.5-7B} and \texttt{Llama-2.5-8B}. While both models focus most of their rules on executing the plan (Step 3), a notable difference emerges in Step 4: Qwen generates significantly more rules corresponding to reviewing or verifying the final answer than Llama. This aligns with recent findings on reasoning behaviors in LLMs~\citep{gandhi2025cognitive}, which identify verification and backward chaining—core to Step 4—as key cognitive abilities underlying a model’s capacity for self-improvement. In their study, Qwen models naturally demonstrate these behaviors, while Llama models initially lack them and only catch up after behaviorally guided training. Our observations extend this insight by revealing that such reflective reasoning tendencies are not only evident in output sequences but also encoded within the internal logic rules learned by the model. The abundance of Step 4 rules in Qwen suggests a deeper inclination toward verification and logical consistency, which may be a crucial factor in its stronger problem-solving performance.
